Accurate Motion Estimation through Random Sample Aggregated Consensus

We reconsider the classic problem of estimating accurately a 2D transformation from point matches between images containing outliers. RANSAC discriminates outliers by randomly generating minimalistic sampled hypotheses and verifying their consensus over the input data. Its response is based on the single hypothesis that obtained the largest inlier support. In this article we show that the resulting accuracy can be improved by aggregating all generated hypotheses. This yields RANSAAC, a framework that improves systematically over RANSAC and its state-of-the-art variants by statistically aggregating hypotheses. To this end, we introduce a simple strategy that allows to rapidly average 2D transformations, leading to an almost negligible extra computational cost. We give practical applications on projective transforms and homography+distortion models and demonstrate a significant performance gain in both cases.

==> coloredAlgo.tex <==
\makeatletter
% code borrowed from Andrew Stacey; See
% http://tex.stackexchange.com/a/50054/3954
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  save picture id/.code={%
    \edef\pgf@temp{#1}%
    \immediate\write\pgfutil@auxout{%
      \noexpand\savepointas{\pgf@temp}{\pgfpictureid}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@#1}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  }
}

\def\savepointas#1#2{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
}

\def\tmk@labeldef#1,#2\@nil{%
  \def\tmk@label{#1}%
  \def\tmk@def{#2}%
}

\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
  \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}\save@orig@pic%
  \pgfsys@getposition{\pgfpictureid}\save@this@pic%
  \pgf@process{\pgfpointorigin\save@this@pic}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@process{\pgfpointorigin\save@orig@pic}%
  \advance\pgf@x by -\pgf@xa
  \advance\pgf@y by -\pgf@ya
  }%
}

% end of Andrew's code

\newlength\AlgIndent
\setlength\AlgIndent{0pt}
% main command to draw the colored background
\newcounter{mymark}
\newcommand\ColorLine{%
  \stepcounter{mymark}%
  \tikz[remember picture with id=mark-\themymark,overlay] {;}%
  \begin{tikzpicture}[remember picture,overlay]%
    \filldraw[red!15!white]%GreenYellow]%
   let \p1=(pic cs:mark-\themymark), 
   \p2=(current page.east)  in 
   ([xshift=-\ALG@thistlm-0.3em,yshift=-0.7ex]0,\y1)  rectangle ++(\linewidth+\AlgIndent,\baselineskip);
  \end{tikzpicture}%
}%

\newcommand\ColorLineTwo{%
  \stepcounter{mymark}%
  \tikz[remember picture with id=mark-\themymark,overlay] {;}%
  \begin{tikzpicture}[remember picture,overlay]%
    \filldraw[green!20!white]%
   let \p1=(pic cs:mark-\themymark), 
   \p2=(current page.east)  in 
   ([xshift=-\ALG@thistlm-0.3em,yshift=-0.7ex]0,\y1)  rectangle ++(\linewidth+\AlgIndent,\baselineskip);
  \end{tikzpicture}%
}%

\newcommand\ColorLineThree{%
  \stepcounter{mymark}%
  \tikz[remember picture with id=mark-\themymark,overlay] {;}%
  \begin{tikzpicture}[remember picture,overlay]%
    \filldraw[black!20!white]%
   let \p1=(pic cs:mark-\themymark), 
   \p2=(current page.east)  in 
   ([xshift=-\ALG@thistlm-0.3em,yshift=-0.7ex]0,\y1)  rectangle ++(\linewidth+\AlgIndent,\baselineskip);
  \end{tikzpicture}%
}%

\newcommand\ColorLineFour{%
  \stepcounter{mymark}%
  \tikz[remember picture with id=mark-\themymark,overlay] {;}%
  \begin{tikzpicture}[remember picture,overlay]%
    \filldraw[red!20!white]%
   let \p1=(pic cs:mark-\themymark), 
   \p2=(current page.east)  in 
   ([xshift=-\ALG@thistlm-0.3em,yshift=-0.7ex]0,\y1)  rectangle ++(\linewidth+\AlgIndent,\baselineskip);
  \end{tikzpicture}%
}%

% colored loops and declarations
\algnewcommand\CREQUIRE{\item[\setlength\AlgIndent{1.6em}\ColorLine\algorithmicrequire]}%
\algnewcommand\CENSURE{\item[\setlength\AlgIndent{1.6em}\ColorLine\algorithmicensure]}%
\algnewcommand\CSTATE{\State\ColorLine}%
\algnewcommand\CSTATETWO{\State\ColorLineTwo}%
\algnewcommand\CSTATETHREE{\State\ColorLineThree}%
\algnewcommand\CSTATEFOUR{\State\ColorLineFour}%
\algnewcommand\CSTATEx{\Statex\ColorLine}%
\algnewcommand\CCOMMENT{\Comment\ColorLine}%

%\def\NoNumber#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}

\algdef{SE}[IF]{CIf}{CEndIf}[1]{\ColorLine\algorithmicif\ #1\ \algorithmicthen}{\ColorLine\algorithmicend\ \algorithmicif}%
\algdef{SE}[FOR]{CFor}{CEndFor}[1]{\ColorLine\algorithmicfor\ #1\ \algorithmicdo}{\ColorLine\algorithmicend\ \algorithmicfor}%
\algdef{SE}[IF]{CIfTwo}{CEndIfTwo}[1]{\ColorLineTwo\algorithmicif\ #1\ \algorithmicthen}{\ColorLineTwo\algorithmicend\ \algorithmicif}%
\algdef{SE}[IF]{CIfThree}{CEndIfThree}[1]{\ColorLineThree\algorithmicif\ #1\ \algorithmicthen}{\ColorLineThree\algorithmicend\ \algorithmicif}%

\algdef{SE}[WHILE]{CWHILE}{ENDWHILE}%
   [2][default]{\ColorLine\algorithmicwhile\ #2\ \algorithmicdo\ALG@compatcomm{#1}}%
   {\algorithmicend\ \algorithmicwhile}%
\algdef{SE}[FOR]{CFOR}{ENDFOR}%
   [2][default]{\ColorLine\algorithmicfor\ #2\ \algorithmicdo\ALG@compatcomm{#1}}%
   {\algorithmicend\ \algorithmicfor}%
\algdef{S}[FOR]{CFORALL}%
   [2][default]{\ColorLine\algorithmicforall\ #2\ \algorithmicdo\ALG@compatcomm{#1}}%
\algdef{SE}[LOOP]{CLOOP}{ENDLOOP}%
   [1][default]{\ColorLine\algorithmicloop\ALG@compatcomm{#1}}%
   {\algorithmicend\ \algorithmicloop}%
\algdef{SE}[REPEAT]{CREPEAT}{UNTIL}%
   [1][default]{\ColorLine\algorithmicrepeat\ALG@compatcomm{#1}}%
   [1]{\algorithmicuntil\ #1}%
\algdef{SE}[IF]{CIF}{ENDIF}%
   [2][default]{\ColorLine\algorithmicif\ #2\ \algorithmicthen\ALG@compatcomm{#1}}%
   {\algorithmicend\ \algorithmicif}%
\algdef{SE}[IF]{CIF}{CENDIF}%
   [2][default]{\ColorLine\algorithmicif\ #2\ \algorithmicthen\ALG@compatcomm{#1}}%
   {\ColorLine\algorithmicend\ \algorithmicif}%
\algdef{C}[IF]{IF}{CELSIF}%
   [2][default]{\ColorLine\algorithmicelse\ \algorithmicif\ #2\ \algorithmicthen\ALG@compatcomm{#1}}%
\algdef{Ce}[ELSE]{IF}{CELSE}{ENDIF}%
   [1][default]{\ColorLine\algorithmicelse\ALG@compatcomm{#1}}%
\algdef{Ce}[ELSE]{IF}{CELSE}{CENDIF}%
   [1][default]{\ColorLine\algorithmicelse\ALG@compatcomm{#1}}%


\makeatother

